Universality and Limitations of Prompt Tuning

Despite the demonstrated empirical efficacy of prompt tuning to adapt a pretrained language model for a new task, the theoretical underpinnings of the difference between "tuning parameters before the input" against "the tuning of model weights" are limited. We thus take one of the first steps to understand the role of soft-prompt tuning for transformer-based architectures. By considering a general purpose architecture, we analyze prompt tuning from the lens of both: universal approximation and limitations with finite-depth fixed-weight pretrained transformers for continuous-valued functions. Our universality result guarantees the existence of a strong transformer with a prompt to approximate any sequence-to-sequence function in the set of Lipschitz functions. The limitations of prompt tuning for limited-depth transformers are first proved by constructing a set of datasets, that cannot be memorized by a prompt of any length for a given single encoder layer. We also provide a lower bound on the required number of tunable prompt parameters and compare the result with the number of parameters required for a low-rank update (based on LoRA) for a single-layer setting. We finally extend our analysis to multi-layer settings by providing sufficient conditions under which the transformer can at best learn datasets from invertible functions only. Our theoretical claims are also corroborated by empirical results.

==> other_files/misc.tex <==
\begin{comment}
\section{Learning Theoretic Bounds}

In the following lemmas, we assume that the classification is done by appending a special token, typically the [CLS] token, to the input sentence. The linear head takes the output embeddings of this [CLS] token to perform the class prediction. \\ 

\begin{lemma}[Informal]
In standard learning theoretic settings, we have the dataset distribution $\D$, the function class $\F$ (here, assume the function class contains the transformer models with a linear head on top for binary classification).
We provide a bound of the following type:
\begin{align}
    \sup_{G \in \F} |\Exp_{x,y \sim \D}[l(G(x,y))] - \frac{1}{m} \sum_{i=1}^{m} [l(G(x_i,y_i))]| \leq \mathcal{K} \label{eq:standard_LT}
\end{align}
Here, $\mathcal{K}$ is the corresponding complexity value, based on rademacher, VC dim etc. We can assume standard conditions on the loss functions - bounded, if needed Lipschitz etc.  \\

Building upon this, we can argue about the following:\\
For the same class $\F$, and inputs coming from the same distribution $\D$:
\begin{enumerate}
    \item we find a prompt $P_G \in \Pm$, per function/model $G$, that minimizes the empirical loss over the sampled dataset.\\
\end{enumerate}
The following type of bound can be provided:

\begin{align}
    \sup_{G \in \F} \inf_{P_G \in \Pm} |\Exp_{x,y \sim \D}[l(G(P_G,x,y))] - \frac{1}{m} \sum_{i=1}^{m} [l(G(P_G,x_i,y_i))]| \leq \mathcal{K'}
\end{align}
Here, $\mathcal{K'}$ is a different complexity term that will be  $\leq \mathcal{K}$. we need to characterize the gap $\mathcal{K} - \mathcal{K'}$ - related to section \ref{sec:min_len_pmt}
\end{lemma}

\textbf{Idea:} The high level is that for each function, we can find the best prompt $P_G$ for it. Then, we can uniformly bound it over the function class.\\

Furthermore, we can have the following :
\begin{lemma}[Informal]
   Using the notation in the previous lemma , we can prove the following:
   \begin{align}
       \inf_{P_G \in \Pm} \frac{1}{m} \sum_{i=1}^{m} [l(G(P_G,x_i,y_i))] \leq \frac{1}{m} \sum_{i=1}^{m} [l(G(x_i,y_i))]
   \end{align}
\end{lemma}
\begin{proof}
    The idea is that we can find a prompt such that the output embedding of [CLS] token has a higher intrinsic dimension, or alternately, higher rank than the case where we don't feed the prompt. Thus, a linear classifier has atleast as good accuracy as without the prompt case.\\
    A useful argument can be borrowed from the paper - \href{https://arxiv.org/pdf/2206.06072.pdf}{here} from eq 8. By appending the prompt $P_G$, we are ensuring that the intrinsic dimension of $(P_G, x)$ is atleast as large as $(x)$ alone, ie $dim(P_G, x) \geq dim(x)$. \\ 
    
    One can then argue that the reduction in rank for $(P_G, x)$ after each layer will not be larger than reduction in rank for $(x)$ alone, based on the use of skip connections. Therefore, the output of the former lies in a larger subspace. \textit{Also, use some arguments from - random projection and sketching literature in linear regression setup} \\
\end{proof}

{\color{red}  \textbf{Note:} This above might help us characterize that prompt-tuning, but with arbitrary length prompt, is atleast as powerful as fine-tuning. Note that theorem 1 and 2 above do not contradict this.  } 


\subsection{Min Length Prompt}
\label{sec:min_len_pmt}
\begin{enumerate}
    \item Given the pretrained model, the pretraining datset, the downstream dataset, and some divergence between pretraining and downstream datasets, can we find the min length prompt so that the above claims hold?
    \item Or more generally speaking, can we say something about the min length prompt?
\end{enumerate}

\subsubsection{Min length prompt to avoid entropy collapse}
Building upon the main theorem of the paper \href{https://arxiv.org/pdf/2303.06296.pdf}{here} and its equation 1. We have that for large $\sigma, n$ the entropy follows $\Omega(n \sigma e^{-\sigma})$. Following a very simple construction procedure, if we add prompt $P$ to input $X$ 









\newpage
\subsection{Accelerated MCMC Sampling - Not a concrete idea yet}
Based on the recent work using in-context learning as approximating the gradient descent for linear models, paper \href{https://arxiv.org/pdf/2211.15661.pdf}{here}, one can extend this to langevin monte carlo for the random variable sampling. More succinctly, we have to carefully construct a prompt (more like in-context learing type). 
We have the following scenario:\\
Given the pretrained transformer model $f$, if we pass the samples from the target distribution $\D_{TX}$ (here $T\rmX$  denotes the marginal for $\rmX$), then the model output distribution $\D^f_{T\rmX}$ and the true output distribution of the labels $\D_{T\rmY|T\rmX}$ will have certain discrepancy which can be quantified using some divergence, possibly KL or Wass (using the frameworks of \href{https://arxiv.org/pdf/2202.05214.pdf}{this paper}). \\
Now, we say that the prompt (as an in-context learning framework) will contain the following $k$ data samples ($k$ just some arbitrary number): $\rmX_i$ and $\f(\rmX_i)$ ($i \in k$) in similar format as theorem 1 at eq 12 in \href{https://arxiv.org/pdf/2211.15661.pdf}{this paper}. What we now argue is that the transformer can perform further Langevin MC steps on top what the input prompt already consists in the form of 
\end{comment}








\begin{comment}
\textbf{Tentative Result 2 (not sure yet): } Assuming that the input data distribution is a mixture, ie, $\D_S = \Sum_{i=1}^{N} \alpha_i \D_i$ , where each $\D_i$ is the input-output tuple $(\rmX, \rmY)$  and $S$ denotes the source/pretraining data, denote the distribution induced by the transformer model $f$,  as $\D^f_S = \sum_{i=1}^{N} \alpha_i \D^f_i$ . \\

Can we argue that the prompt allows the conditional downstream task distribution of the output from the transformer, denote by $\D^f_{T|P=p}$ (where $T$ is the target/downstream task, $P$ is the prompt random variable and $p$ is its realization) , to be close to the conditional $\D^f_{S|P=p}$ , w.r.t some divergence (or distance or even better a metric) say Wass or TVD?\\
Useful to model $\D^f_{S|P=p}$ as a mixture of \textbf{Matrix Normal} distributions - \href{https://en.wikipedia.org/wiki/Matrix_normal_distribution}{link}, where each of the N components is a matrix normal dist. Other useful properties are on page 7 - propostion 1 and 2 \href{https://arxiv.org/pdf/1907.05254.pdf}{here}. \\

\begin{lemma}
    The mixture of Matrix normal distributions (with countably infinite components) is dense in $\mathcal{P}(\mathbb{R}^{n \times d})$ (\mathcal{P} being the set of all prob measures over the space of matrices of size $n \times d$ ) for the Wass-p metric. We consider p as 1, since we are dealing with W1 metric. Also the underlying metric for the Wass is $l(\rmY, \bar{\rmY}) + M \rho_f (f(p, \rmX), f(p, \bar{\rmX})$ , where $M$ is the Lips constant for the loss and $\rho_f$ is the metric for the output of the transformer $f$ (borrowed from page 15 \href{https://arxiv.org/pdf/2304.02064.pdf}{here}). We can consider $\rho_f$ as a matrix norm as well, like the inf or 2 norm.
\end{lemma}

\begin{proof}
    The sketch follows from the Lemma 3.1 on page 7 of the \href{https://arxiv.org/pdf/1907.05254.pdf}{same paper}. By further noting that the matrix normal distibution has a one-one correspondence with the standard multivariate normal distribution (based on the \href{https://en.wikipedia.org/wiki/Matrix_normal_distribution#Definition}{definition}), we finish the proof.
\end{proof}

\textbf{Can we say that the following: } Assume that the input to each layer of the transformer has the exact same support set. Can we say that each layer performs an MCMC type sampling so that the output from the final layer is a random variable that belongs to the desired target distribution? In our prompt case, can we say that the best case prompt allows such a transformation? The Markov Chain is formed by the layer, which is also quite natural for NNs. \\

\end{comment}

